Training neural network ensembles via trajectory sampling

In machine learning, there is renewed interest in neural network ensembles (NNEs), whereby predictions are obtained as an aggregate from a diverse set of smaller models, rather than from a single larger model. Here, we show how to define and train a NNE using techniques from the study of rare trajectories in stochastic systems. We define an NNE in terms of the trajectory of the model parameters under a simple, and discrete in time, diffusive dynamics, and train the NNE by biasing these trajectories towards a small time-integrated loss, as controlled by appropriate counting fields which act as hyperparameters. We demonstrate the viability of this technique on a range of simple supervised learning tasks. We discuss potential advantages of our trajectory sampling approach compared with more conventional gradient based methods.

==> sections/theoretical_expectations.tex <==
\section{Theoretical Expectations}

In the simple linear perceptron problem, we can make predictions about the relationship between the time-averaged expected loss and $s$. When we substitute \er{eq:exact-lp-partition-sum} into \er{eq:partition-function}, find two clear regimes:

\begin{equation}\label{eq:exact-linear-loss-vs-s}
    \mathbb{E}\left[\frac{1}{\tau} \mathcal{L}(\tilde{\omega})\right] \approx 
    \frac{1}{2}\text{tr}( B^T B ) - \frac{1}{2}\text{tr}({C}) -
    \begin{cases}
        \frac{1}{2s\tau}, & \text{for } s\sigma^2 \ll 1 \\
        \frac{1}{2s} & \text{for } s\sigma^2 \gg 1.
    \end{cases}
\end{equation}

\jfm{How much of the derivation for this should we include?}

The first two terms of \er{eq:exact-linear-loss-vs-s} are constants given by samples in the dataset. This also specifies the minimum loss achievable, given the data. When $s\sigma^2 \ll 1$, a dependence on $\frac{1}{\tau}$ emerges, which is responsible for the banding in \fr{fig:linear-s-ensemble-plots} for small values of $s$. A higher value of $\tau$ will lead to a lower loss. However, when $s\sigma^2 \gg 1$, then this banding behaviour disappears, and all values of $\tau$ converge to the same value, for a given $s$.

When $\tau=1$, the conditions in \er{eq:exact-linear-loss-vs-s} become the same, and so is unaffected by $\sigma$. $\sigma$, therefore, only controls where the banding occurs. If the banding is required at $s \gg 1$, choose a small value of $\sigma$ to compensate. This is visually shown in the difference between \fr{fig:linear-s-ensemble-plots} (a) and \fr{fig:linear-s-ensemble-plots} (b), where the first has a smaller value of $\sigma$, which ``moves'' the banding convergence to a higher value of $s$. We see that the banding occurs roughly two orders of magnitude in higher $s$ as $\sigma^2$ is roughly two orders of magnitude smaller.

Now that the banding regime can be controlled by choosing the $\sigma$ parameter, one can also control the loss. One will have the same decrease in loss by doubling $s$, as one would have doubling $\tau$ instead, provided that $2s\sigma^2 \ll 1$. This provides a mechanism for choosing between exploitation vs exploration. Increasing $s$ will increase the exploitation part of the search, while increasing $\tau$ will increase exploration. \jfm{There should be a much better way of phrasing this.}

\jfm{Should we include graphs showing that changing $\sigma$ changes the banding? Additionally, should we introduce noise into the data generated so that we can show a minimum loss?}

\jfm{Mention ``Coupled Replicas''}

% BELOW ARE TODOS WHICH ARE NOW COVERED IN THE PREVIOUS THEORY SECTION

%\jfm{This section can also give some intuition behind choosing the original dynamics, however, I think it is useful to go with the second perspective at first, and then choose $\beta > 0$, which corresponds a valid value of $\sigma$ for the first perspective.}

%\jfm{One perspective is having the original dynamics be a Gaussian process - essentially just a random walk. This allows us to have some very easy perturbative dynamics, which allows us to simply evaluate the acceptance as just $\exp(-s\Delta \mathcal{L})$. It is possible to have another dynamics:}

%\jfm{Second perspective is having the original dynamics be $\tau$ unrelated models which follow neuroevolution - i.e. are weighted by $\exp(-s\mathcal{L}(\params))$. This forms the original ensemble of models which we then tilt to couple the models to their neighbours such that we form a chain/trajectory. This coupling comes in the form of $\exp(-\beta [(\params_{t-1}-\params{t})^2+(\params_{t}-\params{t+1})^2])$.}

%\jfm{Second perspective is exactly equivalent to the first perspective when $\beta \propto \frac{1}{\sigma^2}$. This means that the first perspective is limited to have $\beta>0$ in order to be defined. When $\beta=0$, this is equivalent to having $\sigma \rightarrow \infty$, and hence there is a flat probability of going from one model to the next in the trajectory. Hence, this means that the trajectory is uncoupled and is only defined by the loss observable.}

%\jfm{The second perspective is less useful computationally, since we often want $\beta > 0$. However, from stat mech theory, we can make comparisons to lowering loss with both $s$ and $\beta$ which can be tuned to drop the loss lower, without lowering the temperature. (I am not sure of the graph to put here, but the one that Juan produce with the heatmap and the contour plot I think would be useful.)}

%\jfm{In our numerical results, we have focused on implementing perspective 1 as we are only interested in $\beta > 0$}


